QuantiPhy: A Quantitative Benchmark Evaluating Physical Reasoning Abilities of Vision-Language Models

Understanding the physical world is essential for generalist AI agents. However, it remains unclear whether state-of-the-art vision perception models (e.g., large VLMs) can reason physical properties quantitatively. Existing evaluations are predominantly VQA-based and qualitative, offering limited insight into whether these models can infer the kinematic quantities of moving objects from video observations. To address this, we present QuantiPhy, the first benchmark designed to quantitatively measure a VLM's physical reasoning ability. Comprising more than 3.3K video-text instances with numerical ground truth, QuantiPhy evaluates a VLM's performance on estimating an object's size, velocity, and acceleration at a given timestamp, using one of these properties as an input prior. The benchmark standardizes prompts and scoring to assess numerical accuracy, enabling fair comparisons across models. Our experiments on state-of-the-art VLMs reveal a consistent gap between their qualitative plausibility and actual numerical correctness. We further provide an in-depth analysis of key factors like background noise, counterfactual priors, and strategic prompting and find that state-of-the-art VLMs lean heavily on pre-trained world knowledge rather than faithfully using the provided visual and textual inputs as references when reasoning kinematic properties quantitatively. QuantiPhy offers the first rigorous, scalable testbed to move VLMs beyond mere verbal plausibility toward a numerically grounded physical understanding.

==> sec/tables/tab_parsing-examples1.tex <==
\begin{tabular}{@{} c L{7.5cm} L{4.0cm} L{3.0cm} @{}}
\toprule
\textbf{\#} & \textbf{Question} & \textbf{GT Prior} & \textbf{GT Depth Info} \\
\midrule
1 & What is the length of the slope in cm? & $t=0.6$, ball acc. $= 4.6\text{m/s}^2$ & $t=0\text{s}$, dist. $\text{slope\_far} = 1.8540\text{m}$, dist. $\text{slope\_near} = 1.7010\text{m}$ \\
2 & What is the basketball's distance from the camera at $1.2\text{s}$ in meters? & acc. $= 9.8 \text{m/s}^2$ & $t=1.0\text{s}$, dist. $\text{ball} = 1.4010\text{m}$, $t=1.2\text{s}$, dist. $\text{ball} = 1.5640\text{m}$ \\
3 & What is the basketball's distance from the camera at $1.2\text{s}$ in meters? & acc. $= 9.8 \text{m/s}^2$ & $t=1.0\text{s}$, dist. $\text{ball} = 1.4010\text{m}$, $t=1.2\text{s}$, dist. $\text{ball} = 1.5640\text{m}$ \\
4 & What is the velocity of the ball at the end of the slope in cm/s? & $t=1.4$, ball acc. $= 4.05\text{m/s}^2$ & $t=1.0\text{s}$, dist. $\text{ball} = 1.7790\text{m}$, dist. $\text{slope\_far\_end} = 1.8150\text{m}$ \\
5 & What is the velocity of the soccer ball at $1.5\text{s}$ in m/s? & gravity acc. $= 9.8\text{m/s}^2$ & $t=1.5\text{s}$, dist. $\text{soccer\_ball} = 1.4020\text{m}$ \\
6 & What is the velocity of the tennis ball at $3.4\text{s}$? & gravity acc. $= 9.8\text{m/s}^2$ & dist. $\text{near\_person} = 2.002\text{m}$, dist. $\text{far\_person} = 3.130\text{m}$ \\
7 & What is the acceleration of the red ball at $0.2\text{s}$ in $\text{cm/s}^2$? & diameter of the red ball $= 7\text{cm}$ & $t=0.2\text{s}$, dist. $\text{book} = 1.0995\text{m}$, $t=0.6\text{s}$, dist. $\text{book} = 1.1510\text{m}$ \\
8 & What is the shoulder breadth of the person in cm? & gravity acc. $= 9.8\text{m/s}^2$ & \\
9 & What is the basketball's diameter in cm? & acc. $= 9.8 \text{m/s}^2$ & $t=1.0\text{s}$, dist. $\text{ball} = 1.4010\text{m}$, $t=1.2\text{s}$, dist. $\text{ball} = 1.5640\text{m}$ \\
10 & What is the velocity of the toy at $2.6\text{s}$ in $\text{cm/s}$? & gravity acc. $= 9.8\text{m/s}^2$ & \\
11 & What is the velocity of the toy at $2.6\text{s}$ in $\text{cm/s}$? & gravity acc. $= 9.8\text{m/s}^2$ & \\
12 & What is the diameter of the tennis ball in cm? & gravity acc. $= 9.8\text{m/s}^2$ & dist. $\text{near\_person} = 2.002\text{m}$, dist. $\text{far\_person} = 3.130\text{m}$ \\
13 & What is the length of the wood block in cm? & ruler calibre $= 1\text{cm}$ & \\
14 & What is the acceleration of the astronaut at time $1\text{s}$ in $\text{m/s}^2$? & height of the astronaut $= 2.2\text{m}$ & $t=1\text{s}$, dist. $\text{astronaut} = 23.137\text{m}$ \\
15 & What is the acceleration of the tennis ball at time $1.5\text{s}$ in $\text{m/s}^2$? & diameter of the tennis ball $= 0.17\text{m}$ & \\
16 & What is the diameter(width) of the plant in meters? & acc. of the mug cup before $0.5\text{s} = 9.8\text{m/s}^2$ & \\
17 & What is the velocity of the ball at the end of the slope in cm/s? & $t=1.4$, ball acc. $= 4.05\text{m/s}^2$ & $t=1.0\text{s}$, dist. $\text{ball} = 1.7790\text{m}$, dist. $\text{slope\_far\_end} = 1.8150\text{m}$ \\
18 & What is the diameter of the soccer ball in cm? & gravity acc. $= 9.8\text{m/s}^2$ & dist. $\text{near\_person} = 2.002\text{m}$, dist. $\text{far\_person} = 3.130\text{m}$ \\
19 & What is the distance between two people in cm? & gravity acc. $= 9.8\text{m/s}^2$ & $t=0.60\text{s}$, dist. $\text{near\_person} = 1.5800\text{m}$, dist. $\text{far\_person} = 3.2370\text{m}$ \\
20 & What is the height of the person in cm? & gravity acc. $= 9.8\text{m/s}^2$ & \\
21 & What is the height of the toy in cm? & gravity acc. $= 9.8\text{m/s}^2$ & \\
22 & What is the width of the box in cm? & gravity acc. $= 9.8\text{m/s}^2$ & dist. $\text{near\_person} = 2.002\text{m}$, dist. $\text{far\_person} = 3.130\text{m}$ \\
23 & What is the height of the yellow toy in cm? & gravity acc. $= 9.8\text{m/s}^2$ & $t=0.60\text{s}$, dist. $\text{jar} = 1.9735\text{m}$, dist. $\text{carrot} = 2.6300\text{m}$ \\
24 & What is the basketball's diameter in cm? & acc. $= 9.8 \text{m/s}^2$ & $t=1.0\text{s}$, dist. $\text{ball} = 1.4010\text{m}$, $t=1.2\text{s}$, dist. $\text{ball} = 1.5640\text{m}$ \\
25 & What is the height of the woman in yellow in meters? & walking velocity $= 1.25\text{m/s}$ & \\
26 & What is the length of the speedboat in meters? & sailboat length $= 12\text{m}$ & \\
27 & What is the length of the string in cm? & gravity acc. $= 9.8 \text{m/s}^2$ & $t=0.3\text{s}$, dist. $\text{ball} = 1.7060\text{m}$, $t=0.6\text{s}$, dist. $\text{ball} = 1.3440\text{m}$ \\
28 & What is the displacement of the rolling object from $0\text{s}$ to $0.6\text{s}$ in cm? & $t=0.6$, ball acc. $= 4.6\text{m/s}^2$ & $t=0\text{s}$, dist. $\text{ball} = 1.8180\text{m}$, $t=0.6\text{s}$, dist. $\text{ball} = 1.7288\text{m}$ \\
29 & What is the basketball's distance from the camera at $1.8\text{s}$ in meters? & acc. $= 9.8 \text{m/s}^2$ & $t=0.0\text{s}$, dist. $\text{ball} = 1.3210\text{m}$, $t=1.8\text{s}$, dist. $\text{ball} = 1.5835\text{m}$ \\
30 & What is the velocity of the tennis ball at $3.4\text{s}$? & gravity acc. $= 9.8\text{m/s}^2$ & dist. $\text{near\_person} = 2.002\text{m}$, dist. $\text{far\_person} = 3.130\text{m}$ \\
31 & What is that ball's acceleration at $0.6\text{s}$ in m/s? & gravity acc. $= 9.8 \text{m/s}^2$ & $t=0.3\text{s}$, dist. $\text{ball} = 1.7060\text{m}$, $t=0.6\text{s}$, dist. $\text{ball} = 1.3440\text{m}$ \\
32 & What is the width of the desk in cm? & $t=1.5$, ball acc. $= 3.0\text{m/s}^2$ & $t=0\text{s}$, dist. $\text{cup} = 1.2100\text{m}$, dist. $\text{desk\_left} = 0.8690\text{m}$ \\
33 & What is the length of the slope in cm? & $t=1.5$, ball acc. $= 3.0\text{m/s}^2$ & $t=0\text{s}$, dist. $\text{slope\_far} = 1.3450\text{m}$, dist. $\text{slope\_near} = 1.1040\text{m}$ \\
34 & What is the length of the box in cm? & gravity acc. $= 9.8\text{m/s}^2$ & dist. $\text{near\_person} = 2.002\text{m}$, dist. $\text{far\_person} = 3.130\text{m}$ \\
\bottomrule
\end{tabular}


==> sec/tables/tab_parsing-examples2.tex <==
\begin{tabular}{@{} c c c C{2.0cm} L{5.0cm} C{1.4cm} L{3.2cm} @{}}
\toprule
\textbf{\#} & \textbf{Video Type} & \textbf{Inference Type} & \textbf{GT Posterior} & \textbf{Raw Response} & \textbf{Parsed Value} & \textbf{Model} \\
\midrule
1 & A3MS & DS & 30.8 & Looking at the video frames, I can see a table $\dots$ Length $= 0.1530\text{m} = 15.30\text{cm}$ & 15.30 & Claude-4.5 Sonnet \\
2 & A3SS & DS & 1.565 & $1.5640 \text{m}$ & 1.564 & Claude-4.5 Sonnet \\
3 & A3SS & DS & 1.565 & $[1.5640]$ & 1.564 & CogVLM2 Video \\
4 & A3SS & DD & 208.76 & $[\text{velocity\_at\_the\_end\_of\_the\_slope}]$ $[\text{unit}]$ & None & CogVLM2 Video \\
5 & A3SS & DD & 2.7968 & $1.5 \text{m/s}$ \textbackslash n In the given video, the soccer ball is flying $\dots$ at 1.5 m/s. & 1.5 & Fuyu-8B \\
6 & A3MC & DD & 542.82 & $2.002\text{m/s}$ \textbackslash n In the image, $\dots$ Therefore, its velocity is 2.002m/s. & 2.002 & Fuyu-8B \\
7 & S3SC & SD & 1086.09 & $0.0 \text{cm/s}^2$ & 0 & Gemini-2.5 Flash \\
8 & A2MC & DS & 39 & $39.8 \text{cm}$ & 39.8 & Gemini-2.5 Flash \\
9 & A3SS & DS & 23.2 & $23.9 \text{cm}$ & 23.9 & Gemini-2.5 Pro \\
10 & A2MS & DD & 357 & $0 \text{cm/s}$ & 0 & Gemini-2.5 Pro \\
11 & A2MX & DD & 357 & $-2549 \text{cm/s}$ & 2549 & ChatGPT-5.1 \\
12 & A3MC & DS & 6.7 & $6.5 \text{cm}$ & 6.5 & ChatGPT-5.1 \\
13 & S2MC & SS & 9.9 & $10 \text{cm}$ & 10 & ChatGPT-5 \\
14 & S3SS & SD & 3.604 & $0 \text{m/s}^2$ & 0 & ChatGPT-5 \\
15 & S2SS & SD & 6.129 & $9.8 \text{m/s}^2$ & 9.8 & InternVL-3.5-30B \\
16 & A2MC & DS & 0.075 & $0.05 \text{m}$ & 0.05 & InternVL-3.5-30B \\
17 & A3SS & DD & 208.76 & $[4.05]$ $[\text{m/s}^2]$ & 4.05 & LLaVA-13B \\
18 & A3MX & DS & 17.5 & $[0.31]$ $[0.28]$ & 0.28 & LLaVA-13B \\
19 & A3MX & DS & 325 & $[3.2370]$ $[\text{m}]$ & 3.237 & LLaVA-13B \\
20 & A2MC & DS & 170 & <think>
So, let's try to $\dots$ maybe the person's height is around $170 \text{cm}$. & 170 & MiniCPM-V 4.5-8B \\
21 & A2MX & DS & 14 & $<\text{think}>$ Okay, so I need to $\dots$ If I can determine the time it & None & MiniCPM-V 4.5-8B \\
22 & A3MX & DS & 7.2 & $0.000000000000000000000\dots$ & 0 & Molmo-7B \\
23 & A3MS & DS & 14 & $15.2 \text{cm}$ & 15.2 & Molmo-7B \\
24 & A3SS & DS & 23.2 & $23.9 \text{cm}<|\text{end}|>$ & 23.9 & Phi-3-Mini-128K-Instruct \\
25 & V2MC & DS & 1.71 & Cannot be determined from given information. & None & Phi-3-Mini-128K-Instruct \\
26 & S2MC & SS & 4.8 & $[\text{Value missing due to insufficient information}]$ & None & Phi-3-Mini-128K-Instruct \\
27 & A3SS & DS & 30 & $34.02 \text{cm}$ & 34.02 & Phi-4-Multimodal-Instruct \\
28 & A3MC & DS & 207.9 & $-22.8 \text{cm}$ & 22.8 & Phi-4-Multimodal-Instruct \\
29 & A3SC & DS & 1.5835 & $1.5835 \text{m}$ & 1.5835 & Qwen3-VL-Instruct-8B \\
30 & A3MC & DD & 542.82 & $0.0 \text{m/s}$ & 0 & Qwen3-VL-Instruct-8B \\
31 & A3SS & DS & 4.939 & $0.000000000000000000000\dots$ & 0 & VILA-7B \\
32 & A3MX & DS & 857.9 & $1.2100 \text{m}$ & 1.21 & VILA-7B \\
33 & A3MS & DS & 30.8 & $13450$ & 13450 & SmolVLM-Instruct \\
34 & A3MC & DS & 19.5 & $1.50000000000000004$ & 1.5 & SmolVLM-Instruct \\
\bottomrule
\end{tabular}
